Data Contamination Through the Lens of Time

Recent claims about the impressive abilities of large language models (LLMs) are often supported by evaluating publicly available benchmarks. Since LLMs train on wide swaths of the internet, this practice raises concerns of data contamination, i.e., evaluating on examples that are explicitly or implicitly included in the training data. Data contamination remains notoriously challenging to measure and mitigate, even with partial attempts like controlled experimentation of training data, canary strings, or embedding similarities. In this work, we conduct the first thorough longitudinal analysis of data contamination in LLMs by using the natural experiment of training cutoffs in GPT models to look at benchmarks released over time. Specifically, we consider two code/mathematical problem-solving datasets, Codeforces and Project Euler, and find statistically significant trends among LLM pass rate vs. GitHub popularity and release date that provide strong evidence of contamination. By open-sourcing our dataset, raw results, and evaluation framework, our work paves the way for rigorous analyses of data contamination in modern models. We conclude with a discussion of best practices and future steps for publicly releasing benchmarks in the age of LLMs that train on webscale data.

==> tables/FunctionalCorrectness.tex <==

\begin{table}[!htbp] \centering 
  \caption{Code Forces} 
  \label{} 
\resizebox{\linewidth}{!}{
\begin{tabular}{@{\extracolsep{-2pt}}lcc|cc|cc|cc} 
 & \multicolumn{4}{c|}{{Codeforces}} & \multicolumn{4}{c}{{Project Euler}} \\
 \cline{2-9}
 \cline{2-9}
 \\[-1.8ex] & \multicolumn{2}{c}{\textit{GPT-4}} & \multicolumn{2}{c|}{\textit{GPT-3.5-Turbo}} & \multicolumn{2}{c}{\textit{GPT-4}} & \multicolumn{2}{c}{\textit{GPT-3.5-Turbo}} \\ 
\cline{2-3} \cline{4-5} \cline{6-7} \cline{8-9}
% \\[-1.8ex] & \multicolumn{2}{c}{Functional Correctness}  & \multicolumn{2}{c}{Functional Correctness} \\ 
\\[-1.8ex] & Before Cutoff & After Cutoff & Before Cutoff & After Cutoff & Before Cutoff & After Cutoff & Before Cutoff & After Cutoff \\ 
% \\[-1.8ex] & (1) & (2)\\ 
\hline \\[-1.8ex] 
 Difficulty & 0.085 & 0.208 & 0.118 & 0.231 & 0.145 & 1.000 & 0.165 & 1.000 \\ 
  % & (0.082, 0.087) & (0.186, 0.232) & (0.115, 0.122) & (0.205, 0.261) & (0.104, 0.196) & (0.000, $\infty$) & (0.117, 0.228) & (0.000, $\infty$) \\ 
  & p = 0.000$^{*}$ & p = 0.000$^{*}$ & p = 0.000$^{*}$ & p = 0.000$^{*}$ & p = 0.000$^{*}$ & p = 1.000 & p = 0.000$^{*}$ & p = 1.000 \\  
  & & \\ 
 Github\_Presence & 1.043 & 0.999 & 1.023 & 1.015 & 1.478 & 1.000 & 1.277 & 1.000 \\  
  % & (1.037, 1.049) & (0.986, 1.013) & (1.017, 1.029) & (0.999, 1.031) & (1.131, 1.949) & (0.000, $\infty$) & (0.961, 1.716) & (0.000, $\infty$) \\ 
  & p = 0.000$^{*}$ & p = 0.922 & p = 0.000$^{*}$ & p = 0.066 & p = 0.005$^{*}$ & p = 1.000 & p = 0.100 & p = 1.000 \\ 
  & & \\ 
 Constant & 37,056,799.000 & 33,016.320 & 2,419,019.000 & 9,103.983 & 0.323 & 0.000 & 0.839 & 0.000 \\ 
  % & (29,059,257.000, 47,287,181.000) & (13,652.930, 80,302.830) \\ 
  & p = 0.000$^{*}$ & p = 0.000$^{*}$ & p = 0.000$^{*}$ & p = 0.000$^{*}$ & p = 0.567 & p = 1.000 & p = 0.936 & p = 1.000 \\ 
  & & \\ 
\hline \\[-1.8ex] 
Observations & 168,015 & 11,631 & 166,434 & 11,600 & 765 & 73 & 765 & 73 \\ 
% Log Likelihood & $-$98,176.300 & $-$5,342.657 & $-$92,679.400 & $-$4,561.613 \\  
% Akaike Inf. Crit. & 196,358.600 & 10,691.310 & 185,364.800 & 9,129.226 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{8}{r}{$^{*}$p$<$0.05} \\ 
\end{tabular} }
\end{table} 


==> tables/TagReproduction.tex <==

\begin{table}[!htbp] \centering 
\resizebox{0.8\columnwidth}{!}{%
% \resizebox{\linewidth}{!}{
\begin{tabular}{@{\extracolsep{5pt}}lcc|cc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{GPT-4}} & \multicolumn{2}{c}{\textit{GPT-3.5-Turbo}} \\ 
\cline{2-3} \cline{4-5}
% \\[-1.8ex] & \multicolumn{2}{c}{Functional Correctness}  & \multicolumn{2}{c}{Functional Correctness} \\ 
\\[-1.8ex] & Before Cutoff & After Cutoff & Before Cutoff & After Cutoff \\ 
% \\[-1.8ex] & (1) & (2)\\ 
\hline \\[-1.8ex] 

 Difficulty & 0.431 & 0.826 & 0.497 & 0.739 \\ 
  & (0.400, 0.465) & (0.707, 0.966) & (0.452, 0.547) & (0.619, 0.883) \\ 
  & p = 0.000$^{*}$ & p = 0.017$^{*}$ & p = 0.000$^{*}$ & p = 0.001$^{*}$ \\ 
  & & \\ 
 Github\_Presence & 0.991 & 0.999 & 0.959 & 1.001 \\  
  & (0.977, 1.005) & (0.981, 1.017) & (0.942, 0.976) & (0.980, 1.022) \\ 
  & p = 0.195 & p = 0.888 & p = 0.00001$^{*}$ & p = 0.955 \\ 
  & & \\ 
 % Constant & 310.696 & 1.026 & 56.613 & 1.540 \\ 
 %  & p = 0.000$^{*}$ & p = 0.968 & p = 0.000$^{*}$ & p = 0.545 \\ 
  % & & \\ 
\hline \\[-1.8ex] 
Observations & 24,474 & 6,425 & 24,474 & 6,425 \\  
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.05} \\ 
\end{tabular} 
}
\caption{Tags Reproduction  -- Codeforces} 
\label{tbl:tag_reproduction} 
\end{table} 

==> tables/binomial_FunctionalCorrectness.tex <==

\begin{table}[!htbp] \centering 
  \caption{Pass\@1} 
  \label{} 
\resizebox{\linewidth}{!}{
\begin{tabular}{@{\extracolsep{-2pt}}lcc|cc|cc|cc} 
 & \multicolumn{4}{c|}{{Codeforces}} & \multicolumn{4}{c}{{Project Euler}} \\
 \cline{2-9}
 \cline{2-9}
 \\[-1.8ex] & \multicolumn{2}{c}{\textit{GPT-4}} & \multicolumn{2}{c|}{\textit{GPT-3.5-Turbo}} & \multicolumn{2}{c}{\textit{GPT-4}} & \multicolumn{2}{c}{\textit{GPT-3.5-Turbo}} \\ 
\cline{2-3} \cline{4-5} \cline{6-7} \cline{8-9}
% \\[-1.8ex] & \multicolumn{2}{c}{Functional Correctness}  & \multicolumn{2}{c}{Functional Correctness} \\ 
\\[-1.8ex] & Before Cutoff & After Cutoff & Before Cutoff & After Cutoff & Before Cutoff & After Cutoff & Before Cutoff & After Cutoff \\ 
% \\[-1.8ex] & (1) & (2)\\ 
\hline \\[-1.8ex] 
 Difficulty & 0.084 & 0.204 & 0.115 & 0.228 & 0.145 & 1.000 & 0.165 & 1.000 \\ 
  & (0.082, 0.087) & (0.183, 0.228) & (0.112, 0.119) & (0.202, 0.257) & ($-$0.171, 0.460) & ($-$115,405.900, 115,407.900) & ($-$0.166, 0.497) & ($-$115,405.900, 115,407.900) \\ 
  & p = 0.000$^{*}$ & p = 0.000$^{*}$ & p = 0.000$^{*}$ & p = 0.000$^{*}$ & p = 0.000$^{*}$ & p = 1.000 & p = 0.000$^{*}$ & p = 1.000 \\ 
  & & \\ 
 Github\_Presence & 1.045 & 1.000 & 1.025 & 1.014 & 1.478 & 1.000 & 1.277 & 1.000 \\ 
  & (1.039, 1.051) & (0.986, 1.014) & (1.019, 1.031) & (0.998, 1.030) & (1.206, 1.749) & ($-$82,726.810, 82,728.810) & (0.986, 1.567) & ($-$82,726.810, 82,728.810) \\ 
  & p = 0.000$^{*}$ & p = 0.988 & p = 0.000$^{*}$ & p = 0.081 & p = 0.005$^{*}$ & p = 1.000 & p = 0.100 & p = 1.000 \\ 
  & & \\ 
 Constant & 37,541,216.000 & 36,517.320 & 2,785,763.000 & 9,989.318 & 0.323 & 0.000 & 0.839 & 0.000 \\
  % & (29,444,987.000, 47,895,732.000) & (15,107.710, 88,780.010) & (2,186,846.000, 3,550,635.000) & (3,842.640, 26,109.620) & ($-$3.546, 4.192) & ($-$1,207,455.000, 1,207,455.000) & ($-$3.415, 5.092) & ($-$1,207,455.000, 1,207,455.000) \\ 
  & p = 0.000$^{*}$ & p = 0.000$^{*}$  & p = 0.000$^{*}$ & p = 0.000$^{*}$ & p = 0.567 & p = 1.000 & p = 0.936 & p = 1.000 \\
  & & \\ 
\hline \\[-1.8ex] 
Observations & 6,738 & 1,378 & 6,738 & 1,378 & 765 & 72 & 765 & 72 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{8}{r}{$^{*}$p$<$0.05} \\ 
\end{tabular} }
\end{table} 


==> tables/code_forces/lr_res_4+3.5_FunctionalCorrectnessTest.tex <==

\begin{table}[!htbp] \centering 
  \resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{@{\extracolsep{5pt}}lcc|cc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{GPT-4}} & \multicolumn{2}{c}{\textit{GPT-3.5-Turbo}} \\ 
\cline{2-3} \cline{4-5}
% \\[-1.8ex] & \multicolumn{2}{c}{Functional Correctness}  & \multicolumn{2}{c}{Functional Correctness} \\ 
\\[-1.8ex] & Before Cutoff & After Cutoff & Before Cutoff & After Cutoff \\ 
% \\[-1.8ex] & (1) & (2)\\ 
\hline \\[-1.8ex] 
 Difficulty & 0.085 & 0.208 & 0.118 & 0.231 \\ 
  & (0.082, 0.087) & (0.186, 0.232) & (0.115, 0.122) & (0.205, 0.261) \\
  & p = 0.000$^{*}$ & p = 0.000$^{*}$ & p = 0.000$^{*}$ & p = 0.000$^{*}$ \\ 
  & & \\ 
 Github\_Presence & 1.043 & 0.999 & 1.023 & 1.015 \\ 
  & (1.037, 1.049) & (0.986, 1.013) & (1.017, 1.029) & (0.999, 1.031) \\
  & p = 0.000$^{*}$ & p = 0.922 & p = 0.000$^{*}$ & p = 0.066 \\ 
  & & \\ 
 Constant & 37,056,799.000 & 33,016.320 & 2,419,019.000 & 9,103.983 \\ 
  % & (29,059,257.000, 47,287,181.000) & (13,652.930, 80,302.830) \\ 
  & p = 0.000$^{*}$ & p = 0.000$^{*}$ & p = 0.000$^{*}$ & p = 0.000$^{*}$ \\ 
  & & \\ 
\hline \\[-1.8ex] 
Observations & 168,015 & 11,631 & 166,434 & 11,600 \\ 
% Log Likelihood & $-$98,176.300 & $-$5,342.657 & $-$92,679.400 & $-$4,561.613 \\  
% Akaike Inf. Crit. & 196,358.600 & 10,691.310 & 185,364.800 & 9,129.226 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{2}{r}{$^{*}$p$<$0.05} \\  
\end{tabular} 
}
\caption{\todo{caption needed}} 
\label{tab:cfFunctionalCorrectnessResults} 
\end{table} 


==> tables/project_euler/lr_res_4+3.5_FunctionalCorrectnesTest.tex <==
% todo: if the style guide allows it we may need a pagebreak
\begin{table}[!bhtp] \centering 
  \resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{@{\extracolsep{5pt}}lcc|cc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{GPT-4}} & \multicolumn{2}{c}{\textit{GPT-3.5-Turbo}} \\ 
\cline{2-3} \cline{4-5}
% \\[-1.8ex] & \multicolumn{2}{c}{Functional Correctness}  & \multicolumn{2}{c}{Functional Correctness} \\ 
\\[-1.8ex] & Before Cutoff & After Cutoff & Before Cutoff & After Cutoff \\ 
% \\[-1.8ex] & (1) & (2)\\ 
\hline \\[-1.8ex] 

 Difficulty & 0.145 & 1.000 & 0.165 & 1.000 \\ 
  & (0.104, 0.196) & (0.000, $\infty$) & (0.117, 0.228) & (0.000, $\infty$) \\ 
  & p = 0.000$^{*}$ & p = 1.000 & p = 0.000$^{*}$ & p = 1.000 \\  
  & & \\ 
 Github\_Presence & 1.478 & 1.000 & 1.277 & 1.000 \\  
  & (1.131, 1.949) & (0.000, $\infty$) & (0.961, 1.716) & (0.000, $\infty$) \\ 
  & p = 0.005$^{*}$ & p = 1.000 & p = 0.100 & p = 1.000 \\ 
  & & \\ 
 Constant & 0.323 & 0.000 & 0.839 & 0.000 \\ 
  & (0.007, 15.405) & (0.000, $\infty$) & (0.012, 56.905) & (0.000, $\infty$) \\  
  & p = 0.567 & p = 1.000 & p = 0.936 & p = 1.000 \\ 
  & & \\ 
\hline \\[-1.8ex] 
Observations & 765 & 73 & 765 & 73 \\ 
% Log Likelihood & $-$98,176.300 & $-$5,342.657 & $-$92,679.400 & $-$4,561.613 \\  
% Akaike Inf. Crit. & 196,358.600 & 10,691.310 & 185,364.800 & 9,129.226 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.05} \\ 
\end{tabular} 
}
\caption{\todo{caption}} 
\label{tab:peFunctionalCorrectnessResults} 
\end{table} 

  


==> tables/project_euler/projecteuler_lr_res_gpt4_FunctionalCorrectnessTest.tex <==

\begin{table}[!htbp] \centering 
  \caption{GPT4 Functional Correctness  -- Project Euler} 
  \label{tbl:gpt4_pe_fc} 
\begin{tabular}{@{\extracolsep{5pt}}lcc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{Dependent variable:}} \\ 
\cline{2-3} 
\\[-1.8ex] & \multicolumn{2}{c}{Functional Correctness} \\ 
 & Before Cutoff & After Cutoff \\ 
\\[-1.8ex] & (1) & (2)\\ 
\hline \\[-1.8ex] 
 Difficulty & 0.145 & 1.000 \\ 
  & (0.104, 0.196) & (0.000, Inf.000) \\ 
  & p = 0.000$^{*}$ & p = 1.000 \\ 
  & & \\ 
 Github\_Presence & 1.478 & 1.000 \\ 
  & (1.131, 1.949) & (0.000, Inf.000) \\ 
  & p = 0.005$^{*}$ & p = 1.000 \\ 
  & & \\ 
 Constant & 0.323 & 0.000 \\ 
  & (0.007, 15.405) & (0.000, Inf.000) \\ 
  & p = 0.567 & p = 1.000 \\ 
  & & \\ 
\hline \\[-1.8ex] 
Observations & 765 & 72 \\ 
Log Likelihood & $-$170.511 & $-$0.000 \\ 
Akaike Inf. Crit. & 347.023 & 6.000 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{2}{r}{$^{*}$p$<$0.05; $^{**}$p$<$[0.**]; $^{***}$p$<$[0.***]} \\ 
\end{tabular} 
\end{table} 


==> tables/project_euler/projecteuler_lr_res_gpt_3.5_turbo_FunctionalCorrectnessTest.tex <==

\begin{table}[!htbp] \centering 
  \caption{GPT 3.5 Turbo Functional Correctness  -- Project Euler} 
  \label{tbl:gpt3_pe_fc} 
\begin{tabular}{@{\extracolsep{5pt}}lcc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{Dependent variable:}} \\ 
\cline{2-3} 
\\[-1.8ex] & \multicolumn{2}{c}{Functional Correctness} \\ 
 & Before Cutoff & After Cutoff \\ 
\\[-1.8ex] & (1) & (2)\\ 
\hline \\[-1.8ex] 
 Difficulty & 0.165 & 1.000 \\ 
  & (0.117, 0.228) & (0.000, Inf.000) \\ 
  & p = 0.000$^{*}$ & p = 1.000 \\ 
  & & \\ 
 Github\_Presence & 1.277 & 1.000 \\ 
  & (0.961, 1.716) & (0.000, Inf.000) \\ 
  & p = 0.100 & p = 1.000 \\ 
  & & \\ 
 Constant & 0.839 & 0.000 \\ 
  & (0.012, 56.905) & (0.000, Inf.000) \\ 
  & p = 0.936 & p = 1.000 \\ 
  & & \\ 
\hline \\[-1.8ex] 
Observations & 765 & 72 \\ 
Log Likelihood & $-$140.542 & $-$0.000 \\ 
Akaike Inf. Crit. & 287.084 & 6.000 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{2}{r}{$^{*}$p$<$0.05; $^{**}$p$<$[0.**]; $^{***}$p$<$[0.***]} \\ 
\end{tabular} 
\end{table} 

